How Uncertain Is My Action? Self-Correcting Visual Planning with Frozen World Models

A frozen latent world model combined with sampling-based model predictive control is a visual planner. At deployment, the executed action can depart from the commanded one, and the frozen model has no way to notice. We show that the model can be run in reverse: for any hypothesized actuation shift, it predicts what it should have observed under that shift, and comparing this prediction with what was actually observed quantifies the shift and lets the planner correct itself. Unlike the residual energy, which mixes the shift with the model's own error, the score keeps only the part of the residual that a shift can produce. This shift score detects the shift with a locally optimal test, estimates it with Cramer-Rao error bars, names the dominant generator, and compensates the planner once an alarm fires. On PushT, TwoRoom and OGBench-Cube with a frozen latent world model, measured detection follows the prediction to within 0.05 AUROC. Self-correction raises success from 0.650 to 0.862 on PushT and from 0.378 to 0.432 on the harder Cube task, levels with an oracle that is told the true shift at the same block, better than five common test-time adaptation methods. On a real robotic arm, the score identifies a base-joint offset that no joint encoder registers and reduces the reach error from 36 mm to 3-5 mm, and under shifts drawn at random and sealed before the session, estimates recover 92-94% of the error reduction achieved with the true shift. The broader implication is that a frozen world model can act as a filter by predicting the future, testing action-interface uncertainty and validity, and finally correcting failures.

==> supp_labels.tex <==
\makeatletter
\WarningFilter{hyperref}{Suppressing link with empty target}
\@namedef{r@alg:sp}{{S1}{}{}{}{}}
\@namedef{r@alg:sp@cref}{{[algorithm][1][]S1}{[1][1][]2}{}{}{}}
\@namedef{r@app:analysis}{{S14}{}{}{}{}}
\@namedef{r@app:analysis@cref}{{[section][14][]S14}{[1][23][]24}{}{}{}}
\@namedef{r@app:baselines}{{S12}{}{}{}{}}
\@namedef{r@app:baselines@cref}{{[section][12][]S12}{[1][20][]21}{}{}{}}
\@namedef{r@app:calibration}{{S11}{}{}{}{}}
\@namedef{r@app:calibration@cref}{{[section][11][]S11}{[1][20][]20}{}{}{}}
\@namedef{r@app:delay}{{S5.4}{}{}{}{}}
\@namedef{r@app:delay@cref}{{[subsection][4][5]S5.4}{[1][13][]13}{}{}{}}
\@namedef{r@app:dino}{{S17}{}{}{}{}}
\@namedef{r@app:dino@cref}{{[section][17][]S17}{[1][30][]30}{}{}{}}
\@namedef{r@app:estimate}{{S5.5}{}{}{}{}}
\@namedef{r@app:estimate@cref}{{[subsection][5][5]S5.5}{[1][13][]14}{}{}{}}
\@namedef{r@app:gof}{{S5.8}{}{}{}{}}
\@namedef{r@app:gof@cref}{{[subsection][8][5]S5.8}{[1][16][]16}{}{}{}}
\@namedef{r@app:identification}{{S16}{}{}{}{}}
\@namedef{r@app:identification@cref}{{[section][16][]S16}{[1][29][]29}{}{}{}}
\@namedef{r@app:lie}{{S4}{}{}{}{}}
\@namedef{r@app:lie@cref}{{[section][4][]S4}{[1][6][]6}{}{}{}}
\@namedef{r@app:limitations}{{S20}{}{}{}{}}
\@namedef{r@app:limitations@cref}{{[section][20][]S20}{[1][38][]38}{}{}{}}
\@namedef{r@app:linear}{{S6}{}{}{}{}}
\@namedef{r@app:linear@cref}{{[section][6][]S6}{[1][16][]16}{}{}{}}
\@namedef{r@app:norm}{{S5.1}{}{}{}{}}
\@namedef{r@app:norm@cref}{{[subsection][1][5]S5.1}{[1][8][]8}{}{}{}}
\@namedef{r@app:nuisance}{{S5.3}{}{}{}{}}
\@namedef{r@app:nuisance@cref}{{[subsection][3][5]S5.3}{[1][11][]11}{}{}{}}
\@namedef{r@app:protocol}{{S9}{}{}{}{}}
\@namedef{r@app:protocol@cref}{{[section][9][]S9}{[1][18][]18}{}{}{}}
\@namedef{r@app:rao}{{S5.2}{}{}{}{}}
\@namedef{r@app:rao@cref}{{[subsection][2][5]S5.2}{[1][10][]10}{}{}{}}
\@namedef{r@app:real}{{S18}{}{}{}{}}
\@namedef{r@app:real@cref}{{[section][18][]S18}{[1][30][]30}{}{}{}}
\@namedef{r@app:recovery}{{S5.6}{}{}{}{}}
\@namedef{r@app:recovery@cref}{{[subsection][6][5]S5.6}{[1][14][]14}{}{}{}}
\@namedef{r@app:recovery-details}{{S15}{}{}{}{}}
\@namedef{r@app:recovery-details@cref}{{[section][15][]S15}{[1][25][]26}{}{}{}}
\@namedef{r@app:related}{{S19}{}{}{}{}}
\@namedef{r@app:related@cref}{{[section][19][]S19}{[1][37][]37}{}{}{}}
\@namedef{r@app:shifts}{{S10}{}{}{}{}}
\@namedef{r@app:shifts@cref}{{[section][10][]S10}{[1][19][]19}{}{}{}}
\@namedef{r@app:theory-notes}{{S3}{}{}{}{}}
\@namedef{r@app:theory-notes@cref}{{[section][3][]S3}{[1][3][]3}{}{}{}}
\@namedef{r@fig:cubegrid}{{S7}{}{}{}{}}
\@namedef{r@fig:cubegrid@cref}{{[figure][7][]S7}{[1][26][]27}{}{}{}}
\@namedef{r@fig:supp-pusht-grid}{{S6}{}{}{}{}}
\@namedef{r@fig:supp-pusht-grid@cref}{{[figure][6][]S6}{[1][26][]26}{}{}{}}
\@namedef{r@lem:lan}{{S5.1}{}{}{}{}}
\@namedef{r@lem:lan@cref}{{[lemma][1][5]S5.1}{[1][10][]10}{}{}{}}
\@namedef{r@prop:confusion}{{S5.1}{}{}{}{}}
\@namedef{r@prop:confusion@cref}{{[propositionA][1][5]S5.1}{[1][16][]16}{}{}{}}
\@namedef{r@tab:attr}{{S17}{}{}{}{}}
\@namedef{r@tab:attr@cref}{{[table][17][]S17}{[1][29][]29}{}{}{}}
\@namedef{r@tab:detbase}{{S7}{}{}{}{}}
\@namedef{r@tab:detbase@cref}{{[table][7][]S7}{[1][23][]24}{}{}{}}
\@namedef{r@tab:detect}{{S5}{}{}{}{}}
\@namedef{r@tab:detect@cref}{{[table][5][]S5}{[1][22][]23}{}{}{}}
\@namedef{r@tab:ident}{{S18}{}{}{}{}}
\@namedef{r@tab:ident@cref}{{[table][18][]S18}{[1][29][]29}{}{}{}}
\@namedef{r@tab:persist}{{S13}{}{}{}{}}
\@namedef{r@tab:persist@cref}{{[table][13][]S13}{[1][27][]27}{}{}{}}
\@namedef{r@tab:supp-ablation}{{S14}{}{}{}{}}
\@namedef{r@tab:supp-ablation@cref}{{[table][14][]S14}{[1][27][]28}{}{}{}}
\@namedef{r@tab:supp-dino}{{S19}{}{}{}{}}
\@namedef{r@tab:supp-dino@cref}{{[table][19][]S19}{[1][30][]30}{}{}{}}
\@namedef{r@tab:supp-native}{{S16}{}{}{}{}}
\@namedef{r@tab:supp-native@cref}{{[table][16][]S16}{[1][28][]29}{}{}{}}
\@namedef{r@tab:supp-windows}{{S6}{}{}{}{}}
\@namedef{r@tab:supp-windows@cref}{{[table][6][]S6}{[1][22][]23}{}{}{}}
\makeatother

